Cut Costs, Not Accuracy: LLM-Powered Data Processing with Guarantees

Large Language Models (LLMs) are being increasingly used as a building block in data systems to process large text datasets. To do so, LLM model providers offer multiple LLMs with different sizes, spanning various cost-quality trade-offs when processing text at scale. Top-of-the-line LLMs (e.g., GPT-4o, Claude Sonnet) operate with high accuracy but are prohibitively expensive when processing many records. To avoid high costs, more affordable but lower quality LLMs (e.g., GPT-4o-mini, Claude Haiku) can be used to process records, but we need to ensure that the overall accuracy does not deviate substantially from that of the top-of-the-line LLMs. The model cascade framework provides a blueprint to manage this trade-off, by using the confidence of LLMs in their output (e.g., log-probabilities) to decide on which records to use the affordable LLM. However, existing solutions following this framework provide only marginal cost savings and weak theoretical guarantees because of poor estimation of the quality of the affordable LLM's outputs. We present BARGAIN, a method that judiciously uses affordable LLMs in data processing to significantly reduce cost while providing strong theoretical guarantees on the solution quality. BARGAIN employs a novel adaptive sampling strategy and statistical estimation procedure that uses data and task characteristics and builds on recent statistical tools to make accurate estimations with tight theoretical guarantees. Variants of BARGAIN can support guarantees on accuracy, precision, or recall of the output. Experimental results across 8 real-world datasets show that BARGAIN reduces cost, on average, by up to 86% more than state-of-the-art, while providing stronger theoretical guarantees on accuracy of output, with similar gains when guaranteeing a desired level of precision or recall.

==> recall.tex <==
\begin{figure}
\begin{minipage}{0.325\textwidth}
    \centering
    \includegraphics[width=\linewidth]{exp_figs/RT_varying_T.pdf}
    \caption{Impact of $T$ in RT Queries}
    \label{fig:rt_res_T}
\end{minipage}
\end{figure}

\section{\name{} for RT Queries}\label{sec:rt}
\begin{algorithm}[t]
\begin{algorithmic}[1]
%\Require Desired recall threshold $T$, probability of failure $\delta$, dataset $D$, proxy model $\mathcal{P}$, oracle model $\mathcal{O}$ and oracle budget $k$
%\Ensure A set $A\subseteq D$ such that $\mathds{P}(R_D(A)<T)<\delta$
%\State $P[i]\leftarrow \mathcal{P}(D[i]) \forall x\in D$
%\State $I\leftarrow $ A random sample of $k$ integers in $\{1, ..., n\}$
%\State $L[i]\leftarrow \mathcal{O}(D[i])$
\State $S\leftarrow $ Sample $k$ points from $D$ uniformly at random
\State $\tau\leftarrow T+\frac{\sqrt{\log(1/\delta)}}{2k^+}$\label{alg:thresh_recall:tau}%, either $\tau^E$ or $\tau^C$
\State\Return $\max\{\rho; \rho\in[0, 1], \mathfrak{R}_{S^+}(\rho)\geq \tau\}$
\caption{Naive Algorithm for RT Queries}\label{alg:thresh_recall}
\end{algorithmic}
\end{algorithm}

\if 0
There are multiple knobs at our disposal: (1) how to sample, (2) how to use the sample to decide the cascade threshold and (3) statistical tools used for analysis. 

The most basic solution is to sample 

\fi 
In this section, we present \name{} for performing RT Queries. 
%\subsection{Result Statements and Overview}

\subsection{Naive Approach with Guarantees}\label{sec:rt_naive}
We first consider a naive approach following the general blueprint as the Naive algorithm for PT Queries. We sample points uniformly at random, and follow the two steps of \textit{recall estimation} and \textit{threshold selection}, analogous to Alg.~\ref{alg:thresh_precision}. Recall estimation allows us to esimate, using the observed labels, whether the true recall, $\mathfrak{R}_D(\rho)$, is more than the target or not. Then, during threshold selection, we use recall estimation to choose a cascade threshold whose true recall is at least $T$. 


%First, consider a solution following the first-attempt blue-print in Sec.~\ref{sec:overview}. Such an approach is presented in Alg.~\ref{alg:thresh_recall}, where we first sample a set of points, find an adjusted target, and set the cascade threshold $\rho_S^\tau$ as maximum $\rho$ such that $\mathfrak{R}_S(\rho)\geq \tau$. We find the maximum $\rho$ since the goal is to maximize precision. We want to return as few points as possible while satisfying the recall requirement. 

\textbf{Recall Estimation}. For any threshold $\rho\in[0, 1]$, to estimate recall, we can use Hoeffding's inequality to relate the observed recall to true recall. To do so, define the set $S^+=\{x, x\in S, \mathcal{O}(x)=1\}$ as the set of observed points with positive labels, and denote $k^+=|S^+|$. We have
\begin{proposition}\label{prop:hoef_single_recall}
    For any $\rho\in[0, 1]$ with $\mathfrak{R}_D(\rho)<T$, we have
    \begin{align*}%\label{eq:hoef_delta}
\mathds{P}(\mathfrak{R}_{S^+}(\rho)\geq T+\sqrt{\frac{\log(1/\alpha)}{2k^+}})\leq\alpha, 
\end{align*}
where $\alpha=[0, 1]$ is a confidence parameter.
\end{proposition}
\textit{Proof Sketch}. Observe that $S^+$ consists of $k^+$ random variables sampled i.i.d from $D^+$, so that $\mathds{E}[\mathfrak{R}_{S^+}(\rho)]=\mathfrak{R}_D(\rho)$. Note that use of $S^+$ instead of $S$ is important to the argument, as $\mathds{E}[\mathfrak{R}_{S}(\rho)]\neq \mathfrak{R}_D(\rho)$ because the denominator of $\mathfrak{R}_{S}(\rho)$ is a random variable. Applying Hoeffding's inequality and the fact that $\mathfrak{R}_D(\rho)<T$ proves the result. \qed


\textbf{Threshold Selection}. Next, we use Prop.~\ref{prop:hoef_single_recall} to choose a cascade threshold. This is shown in Alg.~\ref{alg:thresh_recall}, and follows a similar high-level approach to the Naive approach for PT queries. The algorithm first samples a set of points $S$, uses it to calculate the \textit{adjusted target} $\tau$, and returns the largest threshold $\rho$, $\rho\in[0, 1]$, whose observed recall is at least $\tau$. The largest threshold is chosen to maximize precision while meeting the recall target. 

Compared with the Naive algorithm for PT Queries, we observe two differences. First, using Prop.~\ref{prop:hoef_single_recall}, we obtain a single adjusted target $\tau$ to decide if a threshold meets the target recall irrespective of the value of $\rho$ while in Alg.~\ref{alg:thresh_precision}, the adjusted target depends on the value of $\rho$ through $k_\rho$. This is because the recall at a threshold $\rho$ depends on all the positive points (whether with a proxy score more or less than $\rho$) while precision at a threshold $\rho$ depends on only the points with a proxy score more than $\rho$. Second, the algorithm finds the maximum recall across all values in $[0, 1]$ instead of considering a candidate set $\mathcal{E}_M$ as was done for PT Queries. Meanwhile, the number of applications of Prop.~\ref{prop:hoef_single_recall} to decide which values of $\rho$ meet the target does not impact the adjusted target, while in Alg.~\ref{alg:thresh_precision} $\tau_\rho$ depended on $M$. This is due to the fact that the recall function is monotonically decreasing, so the failure of Alg.~\ref{alg:thresh_recall} to meet the target can be attributed to a single event and thus does not require an application of union bound across all thresholds considered, as we discuss in more details below. Note that in practice it is sufficient to check $\rho\in\{S^+\}\cup\{0\}$ instead of $\rho\in[0, 1]$, given that $\mathfrak{R}_{S^+}(\rho)$ anywhere beside points in $S^+$. 

\begin{lemma}\label{lemma:adj_target_hoef}
    Let $\rho_S$ be the cascade threshold found by Alg.~\ref{alg:thresh_recall}. We have $\mathds{P}(\mathfrak{P}_D(\rho_S)<T)\leq \delta.$
\end{lemma}

\textit{Proof Sketch}. Let $\bar{\rho}=\min\{\rho;\rho\in[0, 1], \mathfrak{R}_D(\rho)<T\}$, and note that, because $\mathfrak{R}_D(\rho)$ is monotonically decreasing in $\rho$, Alg.~\ref{alg:thresh_recall} fails to meet the target if an only if $\rho_S\geq\bar{\rho}$. Furthermore, also due to monotonicity of $\mathfrak{R}_D$, we have $\mathfrak{R}_{S^+}(\bar{\rho})\geq\mathfrak{R}_{S^+}(\rho)$ for all $\rho<\bar{\rho}$, so that if $\mathfrak{R}_{S^+}(\rho)\geq \tau$ then $\mathfrak{R}_{S^+}(\bar{\rho})\geq\tau$. As such, Alg.~\ref{alg:thresh_recall} fails to meet the target if only if $\mathfrak{R}_{S^+}(\bar{\rho})\geq\tau$. $\mathds{P}(\mathfrak{R}_{S^+}(\bar{\rho})\geq\tau)\leq \delta$ by Prop.~\ref{prop:hoef_single_recall}, completing the proof. \qed


\if 0
only needs to depend on a single 

This is because recall, as we see below, for 


The following lemma shows that for an appropriately chosen $\tau$, the algorithm satisfies the recall target.


\begin{lemma}\label{lemma:adj_target_hoef}
Alg.~\ref{alg:thresh_recall} meets the target threshold with the desired probability when choosing adjusted target, $\tau$ as 
\begin{align*}
    \tau=T+\sqrt{\frac{\log(1/\delta)}{2k^+}},
\end{align*}
where $k^+$ is the number of positive observed samples.
\end{lemma}

Lemma~\ref{lemma:adj_target_hoef} shows that adjusting the target by $\sqrt{\frac{\log(1/\delta)}{2k^+}}$ leads to a method that satisfies the recall requirements. At a high level, the result holds by bounding the difference between true recall at a proxy threshold, $\rho$, $\mathfrak{R}_D(\rho)$, and observed recall at the threshold, $\mathfrak{R}_S(\rho)$, by $\sqrt{\frac{\log(1/\delta)}{2k^+}}$ using Hoeffding's inequality. This is then used to argue that if we choose a $\rho$ such that its observed recall is more than $T+\sqrt{\frac{\log(1/\delta)}{2k^+}}$, then its true recall is also at least $T$. Although, as we discuss in our detailed proof in Sec. XXX, more theoretical plumbing is needed to make the above argument rigorous (in fact, $\mathfrak{R}_D(\rho)\neq \mathds{E}_{S\sim D}\mathfrak{R}_S(\rho)$, since $\mathfrak{R}_S(\rho)$ is a ratio of two random variables), the analysis does rely on a blackbox application of Hoeffding's inequality to bound the difference between observed and true mean of random variables.

\fi


\subsection{\name{}$_R$-U: Task-Aware Estimation}
Note that recall estimation using Prop.~\ref{prop:hoef_single_recall} relies on Hoeffding's inequality to relate observed recall to true recall. As was also the case for precision estimation, Hoeffding's inequality provides a loose bound on the true recall. As we show below, a much tighter bound is possible by specifically considering the characteristics of recall into account. 
\begin{proposition}\label{prop:exact_single_recall}
    For any $\rho\in[0, 1]$ with $\mathfrak{R}_D(\rho)<T$, we have
    \begin{align*}%\label{eq:hoef_delta}
        \mathds{P}(\mathfrak{R}_{S^+}(\rho)\geq \mathds{T}(T, k^+, \alpha))\leq\alpha,\quad\text{where}
    \end{align*}
    \begin{align*}
        \mathds{T}(T, k^+, \alpha)=\frac{1}{k^+}\min\{\kappa; \kappa\in[k^+], \mathds{P}(\mathcal{B}(k^+, T)\geq\kappa)\leq \alpha\},
    \end{align*}
    and $\mathds{P}(\mathcal{B}(k^+, T)\geq \kappa)$ is the tail probability of a binomial distribution with parameters $k^+$ and $T$.
\end{proposition}
\textit{Proof Sketch}. For any $\rho$ and any of random variables, $x$, $x\in S^+$, 
\begin{align*}
    \mathds{P}(\mathds{I}[\mathcal{S}(x)\geq\rho])=\frac{\sum_{y\in D^+}\mathds{I}[\mathcal{S}(y)\geq\rho]}{|D^+|}=\mathfrak{R}_D(\rho)<T,
\end{align*}
where the first equality is by definition and given that $x$ is a sample uniformly at random from $D^+$.
Furthermore, $\mathfrak{R}_{S^+}(\rho)=\frac{\sum_{x\in S^+}\mathds{I}[\mathcal{S}(x)\geq\rho]}{k^+}$, so that
%The probability $\mathds{P}(\mathds{I}[X_i\geq\rho])$ is bounded as 
%\begin{align*}%\label{eq:bound_tail}
%    \mathds{P}(\mathds{I}[X_i\geq\bar{\rho}_D])< T.
%\end{align*}
%Eq.~\ref{eq:bound_tail} follows the definition of $\bar{\rho}_D$. Specifically, 
%Note that
%by definition of $\bar{\rho}_D$, we have that $\frac{\text{\# positive in}\,[\bar{\rho}_D, 1]}{\text{total \# positives}}<T$. Thus, when uniformly sampling over all positive data points, 
$k^+\times \mathfrak{R}_{S^+}(\rho)$ is the sum of $k^+$ i.i.d Bernoulli random variables with probability of success $\mathfrak{R}_{D}(\rho)$. Consequently, for any $\tau\geq T$, 
$$\mathds{P}(\mathfrak{R}_{S^+}(\rho)\geq \tau)=\mathds{P}(\mathcal{B}(k^+, \mathfrak{R}_D(\rho))\geq k^+\times\tau)\leq \mathds{P}(\mathcal{B}(k^+, T)\geq k^+\times\tau).$$
Setting $\tau=\mathds{T}(T, K^+, \alpha)$, we have $\mathds{P}(\mathcal{B}(k^+, T)\geq k^+\times\tau)\alpha$ by definition, completing the proof.\qed

Our approach, \name{}$_R$-U uses Prop.~\ref{prop:exact_single_recall} and $\mathds{T}$ as the adjusted target, instead of $T+\sqrt{\frac{\log(1/\alpha)}{2K^+}}$ from Prop.~\ref{prop:hoef_single_recall}, and selects the cascade threshold as $\max\{\rho; \rho\in[0, 1], \mathfrak{R}_{S^+}(\rho)\geq \mathds{T}(T, k^+, \delta)\}$. Thus, the approach proceeds similar to Alg.~\ref{alg:thresh_recall}, but replaces the definition of $\tau$ to $\mathds{T}(T, k^+, \delta)$ in Line~\ref{alg:thresh_recall:tau}. \name{}$_R$-U ensure $\mathfrak{R}_D(\rho)\geq T$ with probability $1-\delta$ as desired, following a proof similar to proof of Lemma~\ref{lemma:adj_target_hoef}, but replacing applications of Prop.~\ref{prop:hoef_single_recall} with Prop.~\ref{prop:exact_single_recall}. Note that the tail probability of a binomial distribution, and therefore the function $\mathds{T}$, can be computed exactly by iterating through all the values of $\kappa$. We omit further proof details and pseudocode for \name{}$_R$-U for the sake of space.

\begin{figure}
    \centering
    \begin{minipage}{0.495\linewidth}
        \includegraphics[width=1\linewidth]{figs/bounds_recall.pdf}
        \caption{Computed Adjusted Target}
        \label{fig:recall_target}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\linewidth}
        \includegraphics[width=1\linewidth]{figs/positive_fraction_500.pdf}
        \caption{Fraction of Positive Points at Proxy Score}
        \label{fig:positive_scores}
    \end{minipage}
\end{figure}

Here, we comment on the usefulness of Prop.~\ref{prop:exact_single_recall} compared with Prop.~\ref{prop:hoef_single_recall}. First, note that the proof of Prop.~\ref{prop:exact_single_recall} performs exact computations to calculate $\mathds{P}(\mathfrak{R}_{S^+}(\rho)\geq \tau)$ for any $\tau$,  compared with Prop.~\ref{prop:hoef_single_recall} the uses Hoeffing's inequality to bound the probability. The use of exact computations allows us to provide much tighter upper bounds compared with Prop.~\ref{prop:hoef_single_recall}. To show this, we compare the adjusted targets provided by Props.~\ref{prop:exact_single_recall} and ~\ref{prop:hoef_single_recall} in Fig.~\ref{fig:recall_target}, setting $k^+100$, $\alpha=0.1$ and varying the value of $T$. The figure shows that Prop.~\ref{prop:hoef_single_recall} provides adjusted targets much smaller than Prop.~\ref{prop:hoef_single_recall}. Indeed, when $T\geq0.9$, Prop.~\ref{prop:hoef_single_recall} provides the trivial adjusted target more than 1, which is not useful and implies the Naive algorithm has to always return the entire dataset to achieve the target, yielding low precision. On the other hand, Prop.~\ref{prop:exact_single_recall} provides a meaningful non-trivial bound, significantly improving the precision of the returned set. In Fig.~\ref{fig:recall_target}, we also compare Prop.~\ref{prop:exact_single_recall} with an application of Lemma~\ref{lemma:lb} to this setting. Note that using Lemma~\ref{lemma:lb} does improve Prop.~\ref{prop:hoef_single_recall}, but performs slightly worse than the exact computation by Prop.~\ref{prop:exact_single_recall}. We provide a more detailed discussion of pros and cons of performing exact computation as in Prop.~\ref{prop:exact_single_recall} compared with using distribution-aware concentration bounds, as in Lemma~\ref{lemma:lb} in Sec.~X. 

\if 0
\begin{theorem}\label{thm:adj_target_exact}
Alg.~\ref{alg:thresh_recall} meets the target threshold with the desired probability when choosing adjusted target, $\tau$ as 
\begin{align*}
    \tau=\frac{1}{k^+}\min\{x, q(x)\leq \delta\}
\end{align*}
and $q(x)=\mathds{P}(\mathcal{B}(k^+, T)\geq x)$ is the tail probability of a binomial distribution with parameters $k^+$ and $T$. %That is, $\mathds{P}_{S\sim D}(R_D(\rho^t_S)< T)\leq \delta$ for either choices of $\tau=\tau^C$ or $\tau=\tau^E$.
\end{theorem}

Theorem~\ref{thm:adj_target_exact} shows that by providing a tighter analysis utilizing characteristics of recall, we can significantly improve the utility of the methods. As figure XX, shows we need a much smaller adjustement that  Lemma~\ref{lemma:adj_target_hoef} suggests, so using Theorem~\ref{thm:adj_target_exact} we can set the cascade threshold to much larger values, improving precision.  \sep{add figure showing difference, maybe also add Kang et al}  We note that adusted targets in Lemma~\ref{lemma:adj_target_hoef}  and Theorem~\ref{thm:adj_target_exact} only depend on the number of positives and are data-independent otherwise. 

Intuitively, the crux of the analysis in Theorem~\ref{thm:adj_target_exact} is observing that failure of Alg.~\ref{alg:thresh_recall} only depends on the difference between $\mathfrak{R}_D(\rho)$ and $\mathfrak{R}_S(\rho)$ for $\rho$ values where $\mathfrak{R}_D(\rho)<T$. For such values of $\rho$, we can reformulate observed recall as a binomial random variable with success probability at most $T$ and $k^+$ number of trials, so that we can bound probability of failure with the tail probability of a binomial random variable. The details are presented in Sec. XX. 
\fi

\if 0
\begin{algorithm}[t]
\begin{algorithmic}[1]
\Require Desired recall threshold $T$, probability of failure $\delta$, dataset $D$, proxy model $\mathcal{P}$, oracle model $\mathcal{O}$ and oracle budget $k$
\Ensure A set $A\subseteq D$ such that $\mathds{P}(R_D(A)<T)<\delta$
%\State $P[i]\leftarrow \mathcal{P}(D[i]) \forall x\in D$
%\State $I\leftarrow $ A random sample of $k$ integers in $\{1, ..., n\}$
%\State $L[i]\leftarrow \mathcal{O}(D[i])$
\State $S\leftarrow $ sample $k$ points from $D$ without replacement with distribution $\mathcal{W}$
\State $\rho_S^{\lambda}\leftarrow\max\{\rho; \rho\in [0, 1], \lambda(S, \rho)\geq T\}$
%\State Sort $S$ in increasing order of proxy scores
%\For {$i$ \textbf{in} $\{1, ..., |S|\}$}
    %\State $\hat{\mu}_l\leftarrow$ lower bound on population mean of $$
%     \State $\rho\leftarrow S[i]$
%     \If{$\lambda(S, \rho)<T$}
%        \State \textbf{break}
%     \EndIf
%\EndFor
%\State $\rho_S\leftarrow $ Proxy score for $S[i-1]$
\State\Return $\{x\in D, \mathcal{P}(x)\geq \rho_S^\lambda\}\cup\{x\in S, \mathcal{O}(x)=1\}$
\caption{Discriminator-based selection algorithm}\label{alg:iterative_recall}
\end{algorithmic}
\end{algorithm}
\fi

    
%\textbf{\name{}$_R$-I$^C$}. 

\subsection{\name{}$_R$-P: Task-Aware Sampling}
Finally, we study how to improve upon \name{}$_R$-U by modifying the sampling procedure. Note that Prop.~\ref{prop:exact_single_recall} and consequently \name{}$_R$-U depends on $k^+$, the number of positive samples observed. When sampling data uniformly at random, the fewer the number of observed positive samples, the larger the adjusted target needs to be, and consequently, the worse the final solution utility. Intuitively, to improve the procedure, we would want to modify the sampling strategy to be able to sample more positive labels. Fig.~\ref{fig:positive_scores} shows the c.d.f of proxy scores for positive labels. As we can see, in real-world datasets, positive labels are often distributed around higher proxy scores, significantly so for some datasets such as Tacred and Imagenet. Thus, to improve sampling by attempting to sample more positive scores, it may be tempting to sample more points where the proxy score is higher and less points where proxy scores are small. However, as we show below, doing so while guaranteeing the recall target is met for any possible dataset is not possible. 

\subsubsection{Lower Bound on Utility\nopunct\\}
The lemma below shows that any algorithm that guarantees the target recall is met with probability $\delta$ will have a precision upper bound based on the probability of sampling points with low scores. That is, reducing the probability that points with low scores are sampled can adversely impact the utility of the algorithm.    

%However, doing so is difficult without knowing which data points are likely to be positive. To see this, consider any algorithm that chooses the cascade threshold as one of $\{0\}\cup S^+$, as was done by the Naive method and \name{}$_R$-U, as well as \cite{kang2020approximate}. Note that the observed recall only changes at proxy score values in $S^+$, so that algorithms that set proxy score based on observed recall fall in that category. 
%Indeed, the following Lemma shows that when the total number of positive data points is small compared with the total data size,  without further assumptions on the data, any cascade threshold selection algorithm that provides theoretical guarantees must return a trivial solution frequently. 

\begin{lemma}\label{lemma:recall_rho_must_be_zero_special}
Consider an algorithm, $A$, that samples a set of $k$ points, $S$, i.i.d. and with a p.m.f $W(x)$ for $x\in D$, and returns a cascade threshold $\rho_{S}$. Assume algorithm $A$ meets the recall target $T$, $T\geq 0.5$, on all possible datasets of size $n$ and with $n^+$ positives. Then, for any dataset $D$, algorithm $A$ must have precision $$\mathds{P}(\mathfrak{P}_D(\rho_{S})\geq \frac{n^+}{n})\leq (1-\alpha)^k-\delta,$$
where $\alpha=\sum_{x\in D^{(1-T)n^+}}\mathcal{W}(x)$.
%for any $t\geq\frac{N^+}{2})$ with $\frac{N^+}{2}$-th lowest proxy score and $\alpha_t$ denotes the probability that the algorithm does not sample any point with proxy score in $[0, x_t]$. Specifically, if sampling $k$ points i.i.d, where each point is sampled with probability $W(x)$ where $\mathcal{W}$ is increasing in $\mathcal{S}(x)$, we have $\alpha\leq(1-\frac{(1-T)t}{N})^k$.
\end{lemma}

\textit{Proof Sketch}. The proof shows that if the algorithm achieves precision more than $\frac{n^+}{n}$ with probability more than $(1-\alpha)^k-\delta$ on a dataset $D$, then there exists some other dataset, $\bar{D}$, only differing with $D$ in the label of its first $(1-T)n^+$ points on which the recall is less than $T$ with probability more than $\delta$. At a high level, this holds because, with a high enough probability, the algorithm cannot distinguish between $\bar{D}$ and $D$ given the observed set $S$. Meanwhile, a cascade threshold that achieves high precision in $D$ does not meet the recall target in $\bar{D}$. See Sec. XxX for more details. \qed

Before discussing Lemma~\ref{lemma:recall_rho_must_be_zero_special}, we note that it holds more generally in cases beyond sampling points i.i.d and also holds when not only looking at, $\alpha$, the probability of the first $(1-T)n^+$, but considering the probability of sampling the first $t$ points for any $t\geq (1-T)n^+$ (so that one cannot avoid the bound by setting high $\mathcal{W}$ for the first $(1-T)n^+$ points, and low $\mathcal{W}$ for the points immediately after). We have stated the above special case for simplicity, and we refer the reader to Appx.~XXX for the statement of this more general result and corresponding discussion.  

Lemma~\ref{lemma:recall_rho_must_be_zero_special} is insightful when $n^+$ is much smaller than $n$, that is, when there are few true positives compared with total data size so that $\frac{n^+}{n}$ is small. In such cases, if $(1-\alpha)^k$ is close to one, or alternatively, $\alpha$ is close to zero, then, the algorithm returns very low precision with high probability, yielding low utility. Recall that $\alpha$ is the probability of sampling any of the $(1-T)n^+$ points with the lowest proxy score. If $\mathcal{W}$ is non-decreasing in the proxy score, then $\alpha\leq \frac{(1-T)n^+}{n}$, so that for small $\frac{n^+}{n}$, $\alpha$ will also be small, implying low precision with high probability. This implies the opposite of our intuition that sampling points with higher proxy scores improves utility, leading to the following dilemma: in real-world datasets, positive labels are often present at higher proxy scores, while if our algorithm guarantees that the recall target is met across \textit{all possible dataset}, then sampling points with higher proxy scores more frequently must lead to an algorithm with low precision. 

We note that the above dilemma holds because we provide theoretical guarantees across \textit{all possible datasets}. When $\frac{n^+}{n}$ is small, it is not possible to know which part of the space the positive labels are. Changing the sampling procedure to focus on a part, $A$ of the space instead of $B$ causes fewer in part $B$, and if indeed there are more positives in $B$, the algorithm will have low precision. Nonetheless, relaxing our theoretical guarantees to hold not on all possible datasets, but on datasets that are most frequently encountered in the real world allows us to improve the utility on such datasets. We next present an algorithm that only provides gaurantees under certain conditions that are valid in real-world datasets. 



\if 0


Consequenty,
\begin{align}\label{eq:no_sample_but_more_than_t}
    \mathds{P}(S\cap D^t=\emptyset,\;& \rho_{S, D}\in (x_t, 1])>\delta,
\end{align}
because
\begin{align*}
    \mathds{P}(S\cap D^t=\emptyset,\;& \rho_{S, D}\in (x_t, 1])\\
    &=\mathds{P}(S\cap D^t=\emptyset)-\mathds{P}(S\cap D^t=\emptyset,\; \rho_{S, D}\in [0, x_t])\\
    &>\alpha-(\alpha-\delta)=\delta.
\end{align*}



Furthermore, given that the algorithm is deterministic except for the sampling procedure, the $\mathds{P}(S\cap \bar{D}^t= \emptyset)=\mathds{P}(S\cap D^t= \emptyset)=\alpha$

selected cascade thresholds for both datasets are identical if $S\cap D^i$there are no points sample in $[0, t]$. The algorithm fails on $\bar{D}$, if it does not not return a threshold in [0, t]. 

Recall that we have the probability that the algorithm does not sample a point $[0, t]$ and returns a threshold in $[0, t]$ is bounded by $\alpha-\delta$. Thus, the prob. the algorithm returns a threshold in $[0, t]$ is bounded by $\alpha-\delta$. \qed


Prob. that the alg returns a threshold in [0, t] is at most the p


The probability of that is at least the probability that it does not return threshold in [0, t] and does not sample any point in [0, t]. 


%Below, we first discuss that this is not only a consequence of uniform sampling but an inherent difficulty when the number of positives are much smaller than the total number of samples. Formally,

\begin{lemma}\label{lemma:recall_rho_must_be_zero}
    Consider an algorithm that assigns probability $\mathcal{W}(x)$ for sampling a data point $x\in D$ (where $\mathcal{W}(x)$ potentially depends on $\mathcal{S}(x)$ but not on $\mathcal{O}(x)$), and chooses, based on the set $S$ of $k$ i.i.d samples from $\mathcal{W}$, a cascade threshold, $\rho_S$ from the set $\{0, \mathcal{S}(x_1), ..., \mathcal{S}(x_{k^+})\}$ where $x_1$, ..., $x_k^+\in S^+$. If the algorithm guarantees $\mathds{P}(\mathfrak{R}_D(\rho_S)<T)\leq \delta$ for all datasets $D$, we must also have $\mathds{P}(\rho_S=0)\geq (1-\frac{(1-T)n^+}{N})^k-\delta$ for all datasets $D$. 
\end{lemma}

\textit{Proof.} Assume for the purpose of contradiction that there exists a dataset $D$ with $N^+$ number of positives such that $\mathds{P}_{S~\mathcal{W}}(\mathfrak{R}_D(\rho_S)<T)\leq \delta$ but with $\mathds{P}{S~\mathcal{W}}(\rho_S=0)< (1-\frac{(1-T)N^+}{N})^k-\delta$. Now consider the data point $x_{i_1}, ..., x_{i_{N^+}}\in D$ with the first $N^+$ smallest weights according to $\mathcal{W}$. First, consider the case that at least half of such points have positive labels.  



consider a dataset where $\mathcal{O}(x)=1$ for the $n^+$ points with the lowest $\mathcal{W}$. Now consider such $n^+$ sorted according to their proxy score, and observe that, the probability of sampling any of the $(1-T)\times n^+$ positive points at which the recall is at least $T$  is at most $\frac{(1-T)\times n^+}{N}$. When taking $k$ samples, probably of not sampling any of such positive points is at least $(1-\frac{(1-T)\times n^+}{N})^k$. Assuming the algorithm selects any of such positive points when sampled, the algorithm needs to return 0 with probability at least $(1-\frac{(1-T)\times n^+}{N})^k-\delta$

Lemma~\ref{lemma:recall_rho_must_be_zero} shows that the cascade threshold must be zero frequently, no matter what the sampling strategy is if the number of true positive are small. It also shows that simply modifying the sampling strategy when positive rate is small and  without any further assumptions on the data, does not help improve the quality of solution. We expand on this further in Sec.X, where we specifically discuss why importance sampling, as used by X to address the problem above does not help solve the solution while providing theoretical gauraneees.
\fi 

%Although importance sampling weighs the positive scores more, as we discuss below, it is only beneficial if the model is well-caliberted. Indeed, the approach is sensitive to positive records with low proxy scores, and if the scores cannot be assumed to be well-caliberated, leads to poor results. Below we formalize this statement, and show how we can further improve the results by making assumption about the proxy.  



\subsubsection{Improvements for Real-World Datasets\nopunct\\}
Despite the negative result of Lemma~\ref{lemma:recall_rho_must_be_zero_special}, in practice, we may want to answer RT queries when the number of positive labels is much smaller than the data size. Here, we discuss a methodology on how and when this can be done. Our results in this section depend on how the data is distributed and don't hold for all possible datasets, since as Lemma~\ref{lemma:recall_rho_must_be_zero_special} shows, it is not possible to make such guarantees and return high precision. Instead, we consider the setting where positive labels are sufficiently \textit{dense}, even if they are few in general. To see how, consider the datasets Tacred or Imagenet in Fig.~\ref{fig:positive_scores}. Such datasets are particularly difficult to find cascade thresholds for using uniform sampling. However, as Fig.~\ref{fig:positive_scores} shows, positive labels are present at higher frequency where proxy scores are higher, that is, they are more dense in high proxy scores. Indeed, for such datasets, we can sample all positive points if we only sample points with proxy scores more than $\lambda$, for some dataset dependent $\lambda$ (e.g., $\lambda=0.75$ for Tacred and Onto). However, determining $\lambda$ is difficult without knowing the positive labels. We first discuss the denseness of positive labels more formally, and then proceed to describe how $\lambda$ can be found through sampling. Note that given a value of $\lambda$, we can simply run \name{}$_R$-U but 
only sampling points whose proxy score is more than $\lambda$. If there are no positive labels before $\lambda$, the algorithm correctly identifies a cascade threshold that meets the recall target. 

%the value 0.75 without knowing the proxy scores is difficult 

\textbf{Dense Positive Labels}. Here, we first formalize the notion of \textit{dense positive labels}. Intuitively, this notion is designed to allow us to ignore the long tail of proxy scores that are not expected to have a positive label. More formally, first define \textit{positive density} at a proxy score $\rho$ and with resolution $r$ as $d(\rho, r)=\frac{\sum_{x\in D^{\rho, r}}\mathds{I}[\mathcal{O}(x)=1]}{|D^{\rho, r}|}$ $D^{\rho,r}=\{x;x\in D, \mathcal{S}(x)\in [\rho, \rho+r)\}$. Positive density denotes the fraction of points in $D^{\rho, r}$ that are positive and is a discrete approximation, based on the dataset $D$, to the probability that a sample is positive given proxy score $\rho$,  $\mathds{P}(\mathcal{O}(x)=1|\mathcal{S}(x)=\rho)$ (also known as correctness likelihood \cite{wang2023calibration}). Note that the resolution parameter $r$ is needed since we are measuring a discrete distribution. Now, for a dataset $D$, let $\lambda$ be the smallest proxy score of the points in $D$ with positive labels. We say that dataset $D$ has \textit{dense positive labels} if $d(\rho, r)\geq\beta$ for all $\rho\in[\lambda, 1]$ where $\beta>0$ is the \textit{minimum density of positive labels} in $D$. 

\begin{algorithm}[t]
\begin{algorithmic}[1]
%\Require Desired precision threshold $T$, probability of failure $\delta$, dataset $D$, proxy model $\mathcal{P}$, oracle model $\mathcal{O}$ and oracle budget $k$, sampling step size $s$
%\Ensure A set $A\subseteq D$ such that $\mathds{P}(P_D(A)<T)<\delta$
\State $k_1, k_2\leftarrow k/2$
\State $\delta_1, \delta_2\leftarrow \delta/2$
\State $\rho_{valid}\leftarrow 0$, $\rho\leftarrow 0.5$
\While {$k_1\geq 0$}
    \State $S\leftarrow\emptyset$
    \State $\delta_1\leftarrow\delta_1/2$
    \While{$\mathring{\mathds{L}}(S, \delta_1)\geq\beta$ \textbf{and} $k_1\geq 0$}
        \State Unif. sample from $\{x;x\in D, \rho\leq\mathcal{S}(x)\leq\rho+r \}$ and add to $S$
        \State $k_{1} -= 1$
        \EndWhile
    \If{$\mathring{\mathds{L}}(S, \delta_1)\geq\beta$}
        \State \textbf{break}
    \EndIf
    \State $\rho_{valid}\leftarrow \rho$, $\rho\leftarrow(1+\rho)/2$    
\EndWhile
\State\Return \name{}$_R$-U sampling $k_2$ points over $[\rho_{valid}, 1]$ with $\delta_2$
\caption{\name{}$_R$-I}\label{alg:prism_r_i}
\end{algorithmic}
\end{algorithm}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/prism_rA.pdf}
    \caption{\name{}$_R$-A}
    \label{fig:prism_Ra}
\end{figure}

\textbf{\name{}$_R$-I}. We can leverage the dense positive labels to improve utility. At a high level, dense positive labels imply that in the part of the space where positive labels are present, they are sufficiently dense. As such, if for a proxy score $\rho$, we sample \textit{enough points} with proxy scores in the range $[\rho, \rho+r]$ and observe no positive labels, we can safely assume that there are no positive labels in the range $[0, \rho]$. More formally, at the threshold $\rho$, if we can guarantee that $d(\rho, r)<\beta$, then the denseness of the positive labels implies that there are no positive labels in $[0, \rho]$. As such, our goal is to find the largest $\rho$ such that $d(\rho, r)<\beta$. This can be done through a combination of sampling and search, as described below. 

The algorithm is presented in Alg.~\ref{alg:prism_r_i}, and consists of two stages. The first stage performs binary search on proxy scores to find the largest $\rho$ such that $d(\rho, r)<\beta$. It does so by using $\mathring{\mathds{L}}$, as defined in Prop.~\ref{prop:anytime_lb}, to find an upper bound on $d(\rho, r)$ using the observed samples. If this upper bound is less than $\beta$, it means there are no positive labels in $[0, \rho]$, and the algorithm proceeds to check the density at $(1+\rho)/2$. This continues until the algorithm runs out of sampling budget or if the upper bound on $d(\rho, r)\geq\beta$. Finally, the algorithm uses the largest $\rho$ with $d(\rho, r)<\beta$ and runs \name{}$_R$-U to find a cascade threshold that meets the target in range $[\rho, 1]$. Note the algorithm assigns half of the sampling budget to the binary search and half to find the cascade threshold. It also divides $\delta$ into two and uses half for binary search and half for finding cascade threshold to bound the total probability of failure, as shown below. 

\begin{lemma}\label{lemma:prism_r_i}
    Let $\rho_S$ be the cascade threshold found by Alg.~\ref{alg:prism_r_i}. For any dataset, $D$, with dense positive labels, $\mathds{P}(\mathfrak{P}_D(\rho_S)<T)\leq \delta.$
\end{lemma}

\textit{Proof Sketch}. Consider a dataset $D$ with dense positive labels, and let $\lambda$ be the smallest score of a positive label in $D$. Note that there are two ways Alg.~\ref{alg:prism_r_i} may fail to meet the final recall target (1) if the threshold, $\rho_{valid}$, found is larger than $\lambda$, or (2) if $\rho_{valid}\leq \lambda$ but \name{}$_R$-U fails to return a threshold that meets the target. The probability of the second event is bounded by $\delta_2$ given Lemma XXXX PROB NEED TO STATE LEMMA. For the first event, note that Alg.~\ref{alg:prism_r_i} finds a $\rho_{valid}$ with $\rho_{valid}>\lambda$ only if at the first iteration where $\rho>\lambda$ we have $\mathring{\mathds{L}}(S, \delta_1)<\beta$. This happens with probability $\delta_1$. Thus, the total probability of failure is bounded by $\delta_1+\delta_2=\delta$.\qed


We note that Lemma~\ref{lemma:prism_r_i} show that \name{}$_R$-I meet the target $T$ on datasets with dense positive labels but does not provide guarantees on datasets whose positive labels are not dense. To put this in the context of the upper bound in Lemma~\ref{lemma:recall_rho_must_be_zero_special}, recall that Lemma~\ref{lemma:recall_rho_must_be_zero_special} applies for algorithms that are guaranteed to meet the target on \textit{all possible datasets}. By providing the guarantee only for datasets with dense positive labels,  \name{}$_R$-I avoid the upper bound on the precision, and as we show in our experiments, is able to provide high precision even for datasets with a low number of positive labels. 

Finally, we consider $\beta$ as a user parameter. Although it is possible to set $\beta$ by sampling, doing so, similar to the original problem of finding a suitable cascade threshold, is difficult when the number of positive labels is small. Instead, we provide an alternative formulation to allow users to set these parameters. For a dataset, $D$, not necessarily with dense labels, let $\lambda\in[0, 1]$ be the smallest proxy score such that $d(\rho, r)\geq\beta$ for all $\rho\in[\lambda, 1]$. We have \name{}$_R$-I returns a threshold, $\rho_S$ where $\mathfrak{R}_{D^{\lambda}}(\rho_S)\geq T$ with probability at least 1-$\delta$, where $D^\lambda=\{x;x\in D, \mathcal{S}(x)\geq\lambda\}$. Observe that $\mathfrak{R}_{D^{\lambda}}$ is a generalization of the notion of recall that ignores low probability positive labels. $\beta$ allows the users to decide how low the probability of ignored labels can be. Setting $\beta=0$, we obtain the original problem setting, which as Lemma~\ref{lemma:recall_rho_must_be_zero_special} shows, cannot be solved with good utility when the number of positive labels is low. The users, therefore, can optionally set $\beta>0$ to improve utility while providing a more relaxed guarantee. In our experiments in real-world datasets, we empirically show that a fixed value of $\beta$ both meets the recall requirement and provides good utility. 

%\textcolor{pink_figma}{$\mathds{L}$}
%of dense positive labels play a role in the utility of \name{}$_R$-I.  The resolution parameter should depend on the number of points in the database and should be set to a value such that $d(\rho, r)$ is calculated based on enough number of points (e.g., in the order of hundreds) to avoid large fluctuations as $\rho$ changes. The parameter $\beta$ 


\if 0
Finally, we present algorithm Alg.~\ref{alg:find_lambda} that finds $\lambda$ through sampling. We have

\begin{lemma}\label{lemma:find_lambda}
    If the proxy scores are concentrated, then Alg.~\ref{alg:find_lambda} returns a value, $\lambda$, such that for all $x\in D, \mathcal{P}(x)\leq \lambda$ we have $\mathcal{O}(x)=1$.  
\end{lemma}

Alg.~\ref{alg:find_lambda} follows general estimation strategies discussed in previous algorithms. Its goal is to find the largest $\lambda$ such that there are no positives in $[0, \lambda)$.

Finally, \name{}$_R$-P, combines Alg.~\ref{alg:find_lambda} with Alg.~\ref{XXX}, to first find the region to sample over, and then XXX. 
\fi


%\textbf{Relationship to Calibration}


\if 0

for a dataset $D$, let $\lambda$ be the smallest proxy score of the points with positive labels. For a resolution parameter, $r$ and a tail probability parameter $\omega$, we say the dataset $D$ is dense from $\lambda$ if for any $\rho\in [\lambda, 1]$, the density at $\rho$, $d(\rho)=\frac{\sum_{x\in D^{\rho, r}}\mathds{I}[\mathcal{O}(x)=1]}{|D^{\rho, r}|}$, where 

Generally speaking, the goal is to find a value $\lambda$ such that for all $x\in D$, $x\in[0, \lambda]$ and $\mathcal{P}(x)<\lambda$ we have $\mathcal{O}(x)=0$. For similar reasons as discussed in Lemma~\ref{lemma:recall_rho_must_be_zero}, finding such an $\lambda$ through sampling is difficult without any further assumption. If the true positive rate is smaller, one may require many samples to be able to guarantee, that there are no positives in $[0, \lambda]$ with high probability. 

We present the following assumption on the distribution of positive labels that can allow us to identify what the value of $\lambda$ is through sampling. Specifically, we say that the positives labels are \textit{concentrated with density parameter $q\in[0, 1]$} if, for a given $q$, there exists an $\lambda\in [0, 1]$ such that for all $x\in[0, \lambda)$ $\mathcal{O}(x)=0$ and for all $z\in [\lambda, 1]$ we have $\sum_{x\in D}\frac{\mathds{I}[x\geq z]\mathds{I}[\mathcal{O}(x)=1]}{\mathds{I}[x\geq\lambda]}\geq q$. This assumption means that there are no positive with proxy score less than $\lambda$, and that, the positives are sufficiently dense for proxy scores larger than $\lambda$. The assumption on sufficiently dense positives allows us to distinguish between points in $[0, \lambda]$ and points in $[\lambda, 1].$


\textbf{Concentrated Positive Labels}. Consider the datasets Tacred or Imagenet in Fig.~\ref{positive_dists.pdf}. Such datasets are particularly difficult to find cascade thresholds for using uniform sampling. However, as Fig.~\ref{positive_dists.pdf} shows, proxy scores are much more present in where proxy scores are higher. For instance, sampling a point with a normalized proxy score less than 0.75 in Tacred or Imagenet will not have a positive label, while sampling points with proxy scores close to 1 will lead to many positive samples. Indeed, for such datasets, we can sample all positive points if we only sample points with proxy scores of more than 0.75. However, 
Nonetheless, in practice, one may be interested in using model cascade for scenarios when positive rate is small. This may be possible if one can make further assumptions on the quality of the proxy scores. Intuitively, such assumptions rely on positive samples being concentrated on large proxy scores. The simplest form of such assumption is assuming any model with proxy score below a certain value $\lambda$ does not have a positive label. Such an assumption can simply be combined with Theorem~\ref{thm:adj_target_exact} to provide guarantees whenever the assumption holds. 

However, determining the value of $\lambda$ may be difficult. It requires knowledge about the model (e.g., models may be calibrated differently, and some models may generate smaller values). Below, we discuss a strategy that attempts to estimate a cut-off threshold, if such a threshold exists. 

\fi







\if 0


A natural solution to the problem with importance sampling is to avoid sampling from records with low proxy scores. If one can apriori bound the number of positive records whose proxy score is small, then ignoring records with small proxy scores will not be detrimental to accuracy. This can be done using \textit{clipped importance sampling}. Using some clipping parameter $\lambda$, define
$$
\mathcal{W}_\lambda(x)= \frac{\mathcal{S}(x)}{\sum_{x\in D, \mathcal{S}(x)\geq \lambda}},\; \forall x\in x\in D, \mathcal{S}(x)\geq \lambda.
$$
$\mathcal{W}_\lambda(x)$ defines a p.m.f. over the elements of $D$ whose proxy score is more than $\lambda$. We discuss how to set $\lambda$ later in this section. 
%is less than The accuracy of such a solution depends on how well-calibrated the proxy model is. 


\if 0We first describe an approach that provides gaurantees based on assumptions on model caliberation. We then discuss how such model caliberation assumptions can be validated using sampling.

First, we define a measure of calibration that is intuitive and useful for our setting. XXX CHECK MAYBE THERE IS SOMETHIING LIKE THIS

\begin{definition}
    Consider $\lambda\in [0, n]$ and the subset $\{x_1, ..., x_{i_\lambda}\}$ of $D$ where $i$ is the largest integer such that $\sum_{j=1}^i\mathcal{P}(x)\leq \lambda.$. We say that the proxy model $\mathcal{P}$ is $(\lambda, \beta)$-calibrated with respect to dataset $D$ if for the subset $\sum_{j=1}^{i_\lambda}\mathcal{O}(x_i)\leq \beta+\lambda$.
\end{definition}
\fi

\textbf{\name{}$_R$-P}. Using clipped importance sampling and Theorem~\ref{theorm:importance_sampling}, it is straightforward to show: 
%Intuitively, if proxy scores are taken as probability that a sample is positive, then $(\lambda, \beta)$-calibration means, for a subset of $D$ whose expected number of positive samples is $\lambda$, the actual number of positive samples are at most $\lambda+\beta$. In practice, this notion allows us to bound the number of positive samples with low scores so that we can only perform sampling on elements with high enough proxy scores. The following Lemma states this formally.

\begin{corollary}\label{cor:clamped}
    Assume at most $\gamma$ percent of the positive samples have proxy score at most $\lambda$, that is $$\frac{\sum_{x\in D, \mathcal{S}(x)<\lambda}\mathds{I}[\mathcal{O}(x)=1]}{\sum_{x\in D}\mathds{I}[\mathcal{O}(x)=1]}\leq \gamma.$$ Then, clipped importance sampling using $\mathcal{W}_\lambda$ and using the target $T'=T(1+\frac{\lambda+\beta}{\gamma-(\lambda+\beta)})$ yields an algorithm that meets the target $T$ with probability $\delta$. \sep{change this based on new definition of $\gamma$, $\lambda$}
\end{corollary}

Corollary~\ref{cor:clamped} is a simple extension of Theorem~\ref{theorm:importance_sampling} (note that setting $\lambda, \gamma=0$ we obtain Theorem~\ref{theorm:importance_sampling}), allowing us to avoid sampling records with very low proxy scores. In practice, $\lambda$ and $\gamma$ can be set to very small values, since the goal of the clipped importance sampling is to only ensure that the variance does not explode because of few positive samples with low proxy scores. As we confirm in our experiments, small default values of $\lambda$ and $\gamma$ hold across datasets and models. 

We also note that if the conditions of Corollary~\ref{cor:clamped} cannot be guaranteed, the user is better off using uniform sampling over importance sampling. Indeed, the utility of importance sampling is contingent on the model providing higher scores for positive samples. Since the utility is sensitive to even one case for which this doesn't hold, using importance sampling with no further assumptions on the data often provides trivial bounds. \sep{Maybe we also need to have a version that also estimates $\lambda$, $\gamma$, or maybe we can always start with uniform and switch to clipped?}

%Finally, we also note that one can attempt to estimate $\lambda$ and $\gamma$ using sampling as well. , to avoid assumptions on model calibration an number of ground-truth samples, one can estimate $\beta$ by sampling. This requires dividing the sampling budget into two, $k_1$ and $k_2$ and also choosing an $\lambda$ values. Then, we can use the $k_1$ samples to estimate the total number of positives in $x_1$, .., $x_{i_\lambda}$. Then, we can use $k_2$ samples to estimate a recall threshold. The algorihtm remains the same, but this simply changes the $\beta$ value used in Lemma~\ref{lemma:clamped}. We need to use union bound to gaurantee correctness so $\delta$ has to be divided by two in each case. We can also use this estimate $\gamma$.

\fi


\subsection{Extensions and Discussion}
\textbf{Why not importance sampling}.


\textbf{System Parameters}

\textbf{Exact compute vs concentration bound}

\textbf{binary vs exponential search}



==> revision_letter.tex <==
\twocolumn
\newcommand{\fighyperparam}{fig:hyperparam_AT_rebuttal}
\newcommand{\tabchernoff}{tab:hoef_vs_chernoff_rebuttal}
\newcommand{\chernoffall}{tab:avg_results_rebuttal}
\newcommand{\variance}{tab:avg_variance_rebuttal}
\newcommand{\naivevariant}{tab:naive_vs_naive_witheq9_rebuttal}





\newcommand{\chernoff}{We note that it is possible to use Chernoff's inequality to define the estimation function instead of Hoeffding's. In Appx.~\ref{appx:chernoff} we discuss how the bound can be applied and present results comparing the use of Chernoff's and Hoeffding's inequality. We saw marginal differences between the two and thus present only Hoeffding's inequality here because it is simpler to apply.}

\newcommand{\chernoffappx}{In our naive approach, we can use Chernoff's bound instead of Hoeffding's inequality. This impacts our estimation function, modifying Eq.~\ref{eq:naive_est}. Applying Chernoff's bound~\cite{mitzenmacher2017probability}, we obtain:

\begin{align*}%\label{eq:naive_chernoff}
\hspace*{-10pt}
\mathscr{E}^{\text{Chernoff}}(S, T, \rho, \alpha)=\mathds{I}\big[\mathfrak{P}_S(\rho)\geq T+\sqrt{\frac{2(1-T)\log(1/\alpha)}{|S^\rho|}}\big]. 
\end{align*}
Appx.~\ref{appx:chernoff_prof} shows the derivation of $\mathscr{E}^{\text{Chernoff}}$ form Chernoff's bound~\cite{mitzenmacher2017probability} (which is less straightforward than using Hoeffding's) and its statistical guarantees. % (that are the same as Hoeffding's). 

We next empirically compare this estimator with $\mathscr{E}^{\text{naive}}$ derived from Hoeffding's inequality. To use $\mathscr{E}^{\text{Chernoff}}$, we follow the same naive approach as before (see Eq.~\ref{eq:rho_S_naive}) but replace $\mathscr{E}^{\text{naive}}$ with $\mathscr{E}^{\text{Chernoff}}$. In the following we use Chernoff to refer to the naive method using $\mathscr{E}^{\text{Chernoff}}$ and Hoeffding to the navie methd using $\mathscr{E}^{\text{naive}}$ as presented in Sec.~\ref{sec:pt:naive}. We present the result of the experiments across different quality metrics averaged across all datasets from Sec.~\ref{sec:exp}, for targets $T=0.7$ and $0.9$ in Table~\ref{\tabchernoff}. (Recall that for AT, the utility is cost saved, for PT it is the recall and for RT it is the  precision, similar to Table~\ref{tab:all_res}.) We see that when quality target is 0.9, Chernoff outperforms Hoeffding, but not at target 0.7. Indeed, comparing $\mathscr{E}^{\text{Chernoff}}$ with $\mathscr{E}^{\text{naive}}$ from Eq.~\ref{eq:naive_est}, we observe that $\mathscr{E}^{\text{Chernoff}}$ provides a tighter bound when $T>\frac{3}{4}$ while Eq.~\ref{eq:naive_est} is tighter when $T<\frac{3}{4}$, meaning Chernoff's bound is sharper only when true mean of observations is close to 1, which implies that its application is only beneficial when $T$ is close to 1, whereas Hoeffding's inequality is sharper when $T$ is smaller. Nonetheless, even when $T$ is large (and Chernoff's bound is sharper), \name{} significantly outperforms both bounds as we see in \Cref{\chernoffall} which presents utility of different methods averaged across all datasets from Sec.~\ref{sec:exp} at $T=0.9$. Superior performance of \name{} is not only due to our sharper bounds using \citet{waudby2024estimating}, but also because of our adaptive sampling and selection methods. We note that Sec. 2.3 of \citet{waudby2024estimating} discusses why their proposed estimation method is sharper than Chernoff/Hoeffding bounds, and we provide an informal discussion on why it is so in our Sec.~\ref{sec:stat_tools}.
}

\newcommand{\proofoverview}{Alg.~\ref{alg:iterative_sample_precision} fails to meet the target if $\mathscr{E}^{\text{\name{}}}$ wrongly estimates a threshold meets the target at any iterations of the algorithm. %, which we call a failure event. Thus, we need to ensure that the probability of this failure event is less than $\delta$ in a random run of the algorithm. 
To bound the probability of this event, we ensure that (1) the estimates for any threshold $\rho$ can be wrong with a bounded probability and use this result to show (2) the total probability of making a wrong estimate across all thresholds is bounded by $\delta$. To show (1), observe that every estimate by $\mathscr{E}^{\text{\name{}}}$ for a threshold $\rho$ uses samples taken uniformly from $D^{\rho}$. Thus, the probability that a single estimate is incorrect is bounded by Lemma~\ref{lemma:lb}. Furthermore, the repeated estimation while sampling for the same threshold is accounted for through \cite{waudby2024estimating} which shows that the estimation procedure in Lemma~\ref{lemma:lb} is \textit{anytime valid}, that is, the estimation can be performed repeatedly during sampling, while still providing the same bound on the overall probability of making a wrong estimate (see Lemma~\ref{lemma:_anytime_replace_original}). Then, to show (2), we use Lemma~\ref{lemma:select_eta} which uses the union bound to account for the total probability of making a wrong estimate across all thresholds.}

\newcommand{\naivemain}{We additionally performed experiments using an alternative naive variant that uses Eq.~\ref{eq:select_eta} (with $\eta=0$). This variant performed similarly to the one in Sec.~\ref{sec:pt:naive}; results are presented in Appx.~\ref{exp:additional_naive}.}

\newcommand{\naiveappx}{Here, we consider the alternative naive approach of using Eq.~\ref{eq:select_eta} with $\eta$=0 for threshold selection, instead of Eq.~\ref{eq:naive_sel}. We implemented this approach and observed that it performs almost identically to using Eq.~\ref{eq:naive_sel}. We show the results in \Cref{\naivevariant} which contains the recall for PT queries with $T=0.9$ averaged across all datasets presented in Table~\ref{tab:all_res}. As Fig.~\ref{fig:prec_candidate} shows, precision is, in practice, monotonic in proxy scores, so Eq.~\ref{eq:select_eta} and Eq.~\ref{eq:naive_sel} often end up choosing the same threshold. Overall, \Cref{\naivevariant} shows that modifying the selection procedure alone does not improve utility; the sampling and estimation also need to be improved, as done by \name{}.}

\newcommand{\naivevariance}{Here, we present the standard deviation of the utility of the methods across 50 different runs (runs whose average was presented in Table~\ref{tab:all_res}). Table~\ref{\variance} shows the results, where we compute the standard deviation of the utility of each method for each dataset (i.e., standard deviation corresponding to values in Table~\ref{tab:all_res}), and present the average across datasets in the table. Table~\ref{\variance} shows that \name{} has lower standard deviation than SUPG. To put this in the context of our broader experimental results, we note that Table~\ref{tab:all_res} showed that PRISM often provides an order of magnitude better utility than SUPG; \Cref{\variance} shows that it provides such high utility \textit{with lower variance} than SUPG. }


\newcommand{\calibration}{Note that the use of proxy scores to decide whether to use the proxy or not is beneficial only if the model is well-calibrated \cite{wang2023calibration}, i.e., there is positive correlation between the value of proxy score and probability of correctness of the proxy. Although our guarantees on output quality always hold even when the models are not calibrated, in such cases, the cascade framework is unlikely to provide high utility, e.g., for PT queries, one obtains low recall even though the precision is guaranteed to meet the precision target.}


\newcommand{\paramsettingmain}{Here, we discuss the role of system parameters in \name{}.

\textbf{Number of Candidate Thresholds, $M$}. $M$ controls the number of candidate thresholds \name{}$_A$ and \name{}$_P$ consider. Increasing $M$ (i.e., having more candidate thresholds) increases the chance of finding a threshold with high utility; however, considering many thresholds requires more samples and could be wasteful if most do not improve utility. To understand the trade-offs, note that there are most $\frac{n}{M}$ records between any two consecutive candidate thresholds in $\mathscr{C}_M$ (by definition, see Eq.~\ref{eq:c_M_def}), and that \name{} returns the $i$-th threshold $\rho_i\in \mathscr{C}_M$ when the $i+1$-th threshold, $\rho_{i+1}$ is estimated to not meet the target. If the precision or accuracy of the proxy monotonically increases in the proxy scores (which, according to Fig.~\ref{fig:prec_candidate}, typically holds in practice), then increasing $M$ can lead to choosing a threshold between $\rho_i$ and $\rho_{i+1}$, but not smaller. This means that, for AT queries (similar argument holds for PT queries, see Appx.~\ref{sec:candidate_set}), the fraction of records processed by the proxy can improve by $\frac{1}{M}$ at most, showing diminishing returns as $M$ increases (e.g., any $M>20$ leads to at most $5\%$ increase in utility over $M=20$). So large values of $M$ are unlikely to provide significantly better utility and the cost incurred by sampling more records to evaluate many thresholds when $M$ is large may offset any such gains. We show this empirically in Appx.~\ref{appx:hyperparams} and recommend $M=20$ as the default value. 

\textbf{Minimum Number of Samples per Threshold, $c$}. The parameter $c$ controls the minimum number of samples taken by \name{}$_A$ variants at a threshold before it decides a threshold does not meet the target. If $c$ is too small, the algorithm might prematurely decide a threshold does not meet the target (before having observed sufficient samples), while if $c$ is too large it might spend too many samples at a threshold that does not meet the target, thus wasting samples. Setting $c$ as a small constant fraction of data size ensures that not too many samples are wasted during estimation relative to total processing cost. This is supported by our experiments (see Appx.~\ref{appx:hyperparams}) that show setting $c$ to 1\% to 5\% of data size performs well across datasets, and in general, utility of \name{} is not very sensitive to $c$ as long as it is not very large compared with data size.

\textbf{Tolerance Parameter, $\eta$}. As \name{}$_A$ and \name{}$_P$ variants iterate through candidate thresholds, they terminate after they consider $\eta$ thresholds that do not meet the target (see Eq.~\ref{eq:select_eta}). $\eta$ is a tolerance parameter that can be set based on whether the quality metric is expected to be monotonic or not. That is, whether, after estimating that a threshold $\rho$ does not meet the target, thresholds smaller than $\rho$ are expected to also not meet the target. In real-world datasets, and as discussed in Sec.~\ref{sec:prism_pu:thresh}, this monotonicity property is expected to hold, and as such we set $\eta=0$ by default. Experiments in Appx.~\ref{appx:hyperparams} validate this.}

\newcommand{\systemparamsexp}{Here, we study the impact of hyperparameters, $M, c, \eta$ on \name{}$_A$-A (we observe similar results on other variants) across various datasets. The results are presented in Figure~\ref{\fighyperparam}.

\textbf{Varying $M$}. Results for varying $M$ are shown in Fig.~\ref{\fighyperparam} (a). The results show that very small values of $M$ lead to low utility, while after $M$ reaches a value of around $20$, the utility stabilizes and increasing $M$ further leads to similar utilities. This is in line with the discussion in Sec.~\ref{sec:hyperparam} which shows diminishing returns for increasing $M$ as $M$ gets larger. Low utility for small $M$ is due to the approach not trying enough thresholds, e.g., when $M=1$, \name{} considers only a single threshold, which in many datasets may not meet the accuracy target and thus \name{} has to use the oracle to process all the records. 

\textbf{Varying $c$}. The results for varying $c$ is presented in Fig.~\ref{\fighyperparam} (b). As discussed in Sec.~\ref{sec:hyperparam}, we see that utility improves initially when $c$ increases, by allocating more samples to each threshold to ensure accurate estimates. However, the trend reverses as $c$ increases further, since spending too many samples on thresholds that does not meet the target causes wasting samples. Nonetheless, Fig.~\ref{\fighyperparam} (b) shows that a large range of values of $c$ set as a small fraction of data size provide good utility across datasets.

\textbf{Varying $\eta$}. We next study the impact of $\eta$ from Eq.~\ref{eq:select_eta}. Note that Alg.~\ref{alg:iterative_sample_accurcay} presented for \name{}$_A$-A only considered $\eta=0$ for ease of presentation (since, as we sill, $\eta=0$ is the best performing variant). We extend the algorithm to support $\eta>0$ in Alg.~\ref{alg:iterative_sample_accurcay_w_etha}, where, based on Eq.~\ref{eq:select_eta}, we modify it to consider $\eta$ thresholds that miss the target before returning the final threshold. The results of running this algorithm with various $\eta$ values is presented in Fig.~\ref{\fighyperparam} (c). As the figure shows, the utility decreases with $\eta$, showing that $\eta=0$ provides the highest utility across datasets. As discussed in Sec.~\ref{sec:hyperparam}, if the accuracy of the proxy monotonically decreases as proxy scores deceases, the thresholds smaller than the first threshold that misses the target will also miss the target, so that there is no benefit having $\eta>0$. Meanwhile, $\eta>0$ means each application of the estimation function needs to be more conservative (see Lemma~\ref{lemma:select_eta}), thus providing worse utility.}



\newcommand{\stattools}{To solve the cascade threshold problem through sampling, we need to estimate, based on observed samples, whether a specific threshold meets the quality target. This estimation can be done using classic concentration bounds such as Hoeffding's or Chernoff's inequality. We instead use recent results by \citet{waudby2024estimating} that provide tighter bounds (as discussed in \cite{waudby2024estimating} and empirically validated in our results). Here, we provide an informal overview of the result by \cite{waudby2024estimating} used in our paper. Formal statement of results are presented in Appx.~\ref{sec:statements}.

For a set of i.i.d random variables, $X=\{X_1, ..,. X_k\}$ whose true mean is $\mu$, we would like to estimate, using $X$, whether the true mean is more than a threshold $m$ or not. Theorem 3 of \cite{waudby2024estimating} provides a hypothesis testing approach for this estimate. It specifies a boolean function $\mathscr{T}(m, X, \alpha)$, which, with high probability, is 1 when $\mu$ is at least $m$ and  0 otherwise. \cite{waudby2024estimating} shows that whenever $\mu<m$,  $\mathds{P}\big(\mathscr{T}(m, X, \alpha)=1\big)\leq \alpha$. That is, $\mathscr{T}$ is unlikely to wrongly estimate the mean is more than $m$ when it is not.  
%Here, we present a simplified version of Theorem 3 from \cite{waudby2024estimating} that is used in our methodology. The lemma provides a method to perform the hypothesis test, $\mathscr{T}(m, X)$ of whether the true mean of a sequence of i.i.d random variables $X=\langle X_1, X_2,... X_i\rangle$ is more than a test value $m$ or not. This test is guaranteed to have a false positive probability of at most $\alpha$ for a confidence parameter $\alpha$. That is, 
\begin{lemma}[Informal and Simplified Statement of Theorem 3 by \cite{waudby2024estimating}]\label{lemma:hypothesis_test}
    Consider the set of i.i.d random variables $X$ with mean $\mu$. %Let $X[:j]$ be the first $j$ random variables in $X$. 
    For a confidence parameter $\alpha\in[0, 1]$, and any $\mu<m$, we have
    \begin{align}\label{eq:betting_lb1}
        \mathds{P}\big(\mathscr{T}(m, X, \alpha)=1\big)\leq \alpha,\,\text{where}
    \end{align}    
    \begin{align}\label{eq:betting_lb2}
        \mathscr{T}(m, X, \alpha)\approx\mathds{I}\big[\mathscr{K}(m, X)\geq\frac{1}{\alpha}\big],
    \end{align}    
     %and $\mathscr{K}(m, Y)$, for any sequence $Y=\langle Y_1, ..., Y_k\rangle$ is defined as 
    \begin{align}\label{eq:k_new}
        \mathscr{K}(m, X)\approx\Pi_{i=1}^{k}\Big(1+\frac{(X_i-m)}{\hat{\sigma}_{i-1}}\sqrt{\log(1/\alpha)}\Big),
    \end{align}
    \begin{align*}
        %\mathds{P}(\mu\geq W(x))<\delta W(x)=XXXXX\\
        %\hspace{-13pt}
        \hat{\sigma}_i^2=\frac{1/4+\sum_{j=1}^i(X_j-\hat{\mu}_j)^2}{i+1}, \;\hat{\mu}_i = \frac{1/2+\sum_{j=1}^iX_j}{i+1}.
    \end{align*} 
\end{lemma}
Note that $\approx$ means \textit{we have dropped some of the terms from the definition} to convey high-level intuition (see Appx.~\ref{sec:statements} for exact formulas). Above, $\hat{\sigma}_i^2$ (resp., $\hat{\mu}_i$) is a term analogous to empirical variance (resp., mean). $\mathscr{K}(m, X)$, informally, quantifies whether the sequence of $X_i$ consistently exceeds $m$, when normalized by the variance $\hat{\sigma}_i^2$; larger values show observations exceed $m$ more frequently (thus suggesting $\mu>m$). The use of empirical variance $\hat{\sigma}_i^2$ contrasts with Hoeffding's inequality that only relies on the empirical mean. Taking standard deviation into account significantly improves the bounds when standard deviation is small, as our experiments show (see Sec.~\ref{sec:prec:unif} for comparison).}

\newcommand{\overview}{Our main proposed \name{} variants for each of the queries are shown in Table~\ref{tab:prism_variants}. The variants in the table perform adaptive sampling; for ease of exposition and comparison purposes, we also present other variants (not listed in the table) that perform uniform sampling. All variants take the quality target, $T$, and confidence parameter, $\delta$, as input, while \name{}$_P$-A and \name{}$_R$-A additionally require the oracle budget, $k$, upfront. All methods additionally use other parameters which need not be set by the users and modifying their default values have limited impact on utility. We discuss how these parameters are set in Sec.~\ref{sec:hyperparam}. %As our experiments show, the internal hyperparameters have little impact on utility of the methods with fixed default values working well across dataset, and thus.

\textbf{Use-cases of Variants.} \name{}$_A$ is suitable for multi-class classification, as well as binary classification without a maximum oracle budget constraint but when the goal is to minimize the total budget used. \name{}$_P$ and \name{}$_R$ on the other hand respect a maximum oracle budget and thus are useful when user wants to stay within a budgetary constraint. Moreover,  \name{}$_P$ and \name{}$_R$ are useful for binary classification tasks with class imbalance, e.g., when there is expected to be few records in the positive class, while \name{}$_A$ is additionally applicable when classes are balanced. Finally, \name{}$_A$-A and \name{}$_A$-M differ in that \name{}$_A$-A chooses a single cascade threshold for {\em all} output classes while \name{}$_A$-M chooses a cascade threshold {\em per class}. As such, \name{}$_A$-M is beneficial if the proxy is differently calibrated for different output classes, which may occur if it is more difficult to correctly estimate one class but not another.}

We thank all reviewers for their comments. We have addressed all of the comments from the reviewers in the paper according to our revision plan, with text \rone{in blue addressing comments from R1}, \rtwo{in green addressing comments from R2}, \rthree{in purple addressing comments from R3} and \rall{in red addressing comments that overlap across reviewers}. We use this same color coding here as well when we directly cite revised content of the paper to distinguish from additional commentary. For each reviewer comment, we discuss the revisions we made (under \textit{Revision Performed}), and for ease of reference, we also include the revision item we had proposed to do in our revision plan (under \textit{Proposed Revision Item}). {\bf \em We have done all the revisions we proposed to do.} We provide a summary of major changes below, and describe them in detail in Secs.~\ref{sec:r1}-\ref{sec:r3}.

\noindent\textbf{Summary of major changes}. In this revision, we have:
\vspace{-0.1cm}
\begin{itemize}%[leftmargin=1.5em]%, labelsep=0.3em]
    \item Added Sec.~\ref{sec:stat_tools}, a new section discussing statistical tools used and high-level intuition behind them. We have also modified Sec.~\ref{sec:pt} and Sec.~\ref{sec:discussion} to refer back to this result and reduced redundancy.
    \item Added Sec.~\ref{sec:overview_outline}, an overview section to outline the proposed methods, discuss their main parameters and use-cases.
    \item Added Sec.~\ref{sec:hyperparam} to discuss how to set parameters in \name{}, and new experiments in Appx.~\ref{appx:hyperparams} to discuss the role of the parameters.
    \item Added new discussion and experiments considering alternative naive approaches, using Chernoff bound in Appx.~\ref{appx:chernoff} and using a different threshold selection method in Appx.~\ref{exp:additional_naive}.
    \item Added new experiments showing standard deviation of the methods in Appx.~\ref{appx:variance_exp}.
    \item Added additional discussions throughout the paper on model calibration, overview of our proofs, and applications of \name{}.
\end{itemize}

%\vspace{-0.2cm}
\section{Response to Reviewer 1}\label{sec:r1}
\vspace{-0.5em}%\vspace{-0.05cm}
\begin{revcomment}{R1O3 (i)}
\textit{``The naive algorithm is analyzed using a Hoeffding bound. Why not a Chernoff bound ...?''}
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a summary of the comparison between Hoeffding's and Chernoff's inequality in the main paper with details and experimental results in our appendix.''

\noindent\textit{Revision Performed:} We have included the comparison between Chernoff and Hoeffding's inequality. As now mentioned in Sec.~\ref{sec:pt:naive}, ``\rone{\chernoff{}}'' Detailed discussion and results are in Appx.~\ref{appx:chernoff}, presented below for ease of reference:  

\begin{table}[h]
\hspace{-0.7cm}
\begin{minipage}{0.51\columnwidth}
    \centering
    \rone{\begin{tabular}{c c c}
    \toprule
        \textbf{Metric} & \textbf{Chern.} & \textbf{Hoeff.}\\\midrule
        AT@0.7 & 52.6 & 52.8\\
        AT@0.9 & 24.3 & 22.9\\
        \hline
        PT@0.7 & 45.3  & 46.9\\
        PT@0.9 & 22.6 & 22.1\\
        \hline
        RT@0.7 & 34.4 & 34.0\\
        RT@0.9 & 30.6 & 25.7  \\ \bottomrule
    \end{tabular}}
    \caption{\rone{Obtained utility from Hoeffding and Chernoff}}
    \label{tab:hoef_vs_chernoff_rebuttal}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}{0.48\columnwidth}
\centering
\rone{
    \begin{tabular}{c c c c}
    \toprule
        \textbf{Method} & \textbf{AT} & \textbf{PT}& \textbf{RT}\\\midrule
        \textbf{SUPG} & 27.8 & 46.7 & 36.5\\
        \textbf{Hoeff.} & 22.9 & 22.1 & 25.7\\
        \textbf{Chern.} & 24.3 & 22.6 & 30.6\\
        %\textbf{PRISM$_*^{U/M}$} & 56.8 & 33.3 & 38.9\\
        \textbf{PRISM$_*$-A} & \textbf{60.5} & \textbf{74.6} & \textbf{44.5}\\\bottomrule
    \end{tabular}}
    \caption{\rone{Utility of different methods given quality target $T=0.9$ across queries}}
    \label{tab:avg_results_rebuttal}
\end{minipage}
\vspace{-0.2cm}
\end{table}

\textit{In Appx.~\ref{appx:chernoff}}: 
\rone{\chernoffappx{}}



\begin{revcomment}{R1O3 (ii)}
\textit{``Many of the methods make use of hypothesis testing ...  shouldn't the analysis account for this?''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include an overview of our proofs in the paper ...''

\noindent\textit{Revision Performed:} Our proofs indeed account for performing multiple hypothesis tests, and we have now included an overview of our proofs in Sec.~\ref{sec:prec:adap} (also addressing R1O3 (iv)) that explains why. To summarize, our proofs account for performing multiple hypothesis tests by using (1) a union bound to account for performing multiple tests when making estimates for different candidate thresholds in Lemma~\ref{lemma:select_eta}, and (2) the results of \citet{waudby2024estimating} to account for performing multiple tests when making multiple estimates for a single candidate threshold. Regarding the latter, the guarantees of \cite{waudby2024estimating}  show the hypothesis tests we perform are \textit{anytime valid}. That is, \cite{waudby2024estimating} bounds the probability of making incorrect estimates when repeatedly estimating while sampling new points. We summarize this dscussion in the newly added proof overview in Sec.~\ref{sec:prec:adap}, which we present here as well for ease of reference:

\textit{In Sec.~\ref{sec:prec:adap}}: \rone{\proofoverview{}}

\begin{revcomment}{R1O3 (iii)}
\textit{``Eq. 9 is what I'd consider the naive approach (with eta=0) ... did it happen in experiments that both methods give different results.''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a discussion of the requested result in the paper and include the experimental results in the Appendix.''

\noindent\textit{Revision Performed:} We have now included results for the requested variants, showing that the requested naive variant performs similarly to the one already presented in the paper. As now discussed in Sec.~\ref{sec:exp:setup}: ``\rone{\naivemain{}}'' We present Appx.~\ref{exp:additional_naive} below for ease of reference.

%\textit{In :} \naivemain{}

\textit{In Appx.~\ref{exp:additional_naive}:} \rone{\naiveappx{}}

\begin{table}[h]
\centering
    \rone{\begin{tabular}{c c}
        \toprule\textbf{Method} & \textbf{Observed Recall} \\\midrule
         Naive & 22.098 \\
         Naive with Eq.~\ref{eq:select_eta} &  22.149\\
        \bottomrule
    \end{tabular}}
    \caption{\rone{PT Query with $T=0.9$}}
    \label{tab:naive_vs_naive_witheq9_rebuttal}
\end{table}

\begin{revcomment}{R1O3 (iv)} \textit{``The adaptive methods produce new samples biased by ... prior samples, ... It's not clear to me whether this is appropriately accounted for.''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include an overview of our proofs in the paper...''

\noindent\textit{Revision Performed:} Our proofs indeed account for performing adaptive sampling, and we have now included an overview of our proofs in Sec.~\ref{sec:prec:adap} (also addressing R1O3 (ii)) that explains why. To summarize, our analysis accounts for the adaptive sampling because the estimation in \name{}, for any threshold $\rho$, is always performed on a uniform sample from $D^\rho$; even though the adaptivity of \name{} means it takes different uniform samples for different thresholds. Because the samples used to estimate for any specific threshold are uniform,  Lemma~\ref{lemma:lb} is used to bound the probability of failure.  The proof overview presents the above discussion in Sec.~\ref{sec:prec:adap}. Our response to R1O3 (ii) includes Sec.~\ref{sec:prec:adap} (please see R1O3 (ii), paragraph \textit{In Sec.~\ref{sec:prec:adap}}: ...) and we omit it here to avoid repetition. 

%\textit{In Sec.~\ref{sec:prec:adap}}: \rone{\proofoverview{}}

\begin{revcomment}{R1O3 (v)} \textit{``The experimental results are averaged over 50 runs. Why is this? ... Was it variance?...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a discussion on why we perform repeated runs in the paper. Moreover, as suggested by R1M1, we will explicitly present which methods met the quality target empirically, and include the methods' variance in the appendix.''

\noindent\textit{Revision Performed:} We now mention in Sec.~\ref{sec:exp:setup} that ``\rone{We performed 50 runs to empirically evaluate whether the methods meet the quality target with the desired probability.}'' To elaborate, performing repeated runs is essential since our guarantees are probabilistic and repeated runs must be performed to evaluate whether the guarantees hold in practice, as
was also done in [21]. In our experiments, to evaluate whether a method met the quality target with the desired probability, we checked whether at least 1-$\delta$ fraction of the runs met the
target, which requires repeated runs. Furthermore we modified Table~\ref{tab:all_res} to show which methods did not meet the quality target empirically (only SUPG on Onto dataset). Additionally, as noted in Sec.~\ref{sec:exp:setup}, ``\rone{We also report observed variances across the 50 runs in Appx.~\ref{appx:variance_exp}; our results show \name{} has lower variance than SUPG}.'' We present Appx.~\ref{appx:variance_exp} below for ease of reference:


\textit{In Appx.~\ref{appx:variance_exp}}: \rone{\naivevariance{}}

\begin{table}[h]
\centering
    \rone{\begin{tabular}{c c c c}
    \toprule
        \textbf{Method} & \textbf{AT} & \textbf{PT}& \textbf{RT}\\\midrule
        \textbf{SUPG}  & 4.7 & 3.3 & 13.7\\
        \textbf{Naive}  & 1.9 & 1.6& 0.7\\
        %\textbf{PRISM$_*^{U/M}$} & 56.8 & 33.3 & 38.9\\
        \textbf{PRISM$_*$-A}  & 3.7 & 2.1& 8.0\\\bottomrule
    \end{tabular}}
    \caption{\rone{Standard deviation of utility of different methods given target $T=0.9$ averaged across datasets}}
    \label{tab:avg_variance_rebuttal}
\end{table}

\begin{revcomment}{R1O3 (vi)} \textit{''... There seems to be some implicit calibration assumption that higher proxy probabilities typically mean higher quality...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a discussion on calibration in the paper, explicitly noting the dependence of utility of our method on model calibration. ''

\noindent\textit{Revision Performed:} We have included a discussion on calibration in Sec.~\ref{sec:background:cascade}, noting the dependence of utility, but not our guarantees (which always hold), on model calibration. Specifically, we mention ``\rone{\calibration{}}''


\begin{revcomment}{R1O1} \textit{``The method uses quite a number of hyperparameter ... it's unclear how they have been chosen''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will extend our experimental analysis to consider other hyperparameters: $\eta$ in PT and $c$ in AT queries. We will show how they impact performance and how to set them. ''

\noindent\textit{Revision Performed:} We have now added Sec.~\ref{sec:hyperparam} to discuss the impact of various system parameters and discuss how to set them. We have furthermore conducted experiments that show the impact of hyperparameters on our methods. The results show our approaches are not sensitive to the hyperparameters, and using fixed default values works well across datasets. The detailed experiments are presented in Appx.~\ref{appx:hyperparams}, and we have included a summary of the results in Sec.~\ref{sec:exp:user_param}.  For ease of reference, we present the discussion from Sec.~\ref{sec:hyperparam} on the role of the parameters and how to set them---as well as the empirical results from Appx.~\ref{appx:hyperparams} below. 


\textit{In Sec.~\ref{sec:hyperparam}}: \rone{\paramsettingmain{}}






\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{exp_figs/res_hyperparams.pdf}
    \caption{\rone{Impact of $M$, $c$ and $\eta$ on \name{}$_A$-A}}
    \label{fig:hyperparam_AT_rebuttal}
\end{figure}

\textit{In Appx.~\ref{appx:hyperparams}}: \rone{\systemparamsexp{}}



\begin{revcomment}{R1O2}
\textit{``The writing is dense ... the paper would benefit from (i) focusing on key points at a higher level ... and (ii) outsourcing everything else to the appendix ... This may also reduce repetitiveness ...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a summary of our methods upfront (based on R3O1-O3), and reduce repetitions.'' 

\noindent\textit{Revision Performed:} We have now modified the paper to (1) include an overview of the methods in Sec.~\ref{sec:overview_outline}, (2) discuss a high-level overview of statistical tools in Sec.~\ref{sec:stat_tools} and (3) reduced repetition and simplified the discussion on how they are applied in Secs.~\ref{sec:pt} and \ref{sec:discussion}. Specifically, the newly added Sec.~\ref{sec:stat_tools} now presents an overview of the statistical results of \cite{waudby2024estimating} used in the paper, focusing on the high-level intuition behind the results and deferring the exact statement to the appendix. Using this formulation, we have then reduced the repetition when discussing how the statistical tools are used Secs.~\ref{sec:pt} and \ref{sec:discussion}. For example, the definitions of $\mathscr{E}^{\text{\name{}}}$, $\mathscr{E}_A^{\text{\name{}}}$ and $\mathscr{E}_R^{\text{\name{}}}$ are much less repetitive, only showcasing the high-level differences between the definitions. Please see the changes marked in \rall{red} in Secs.~\ref{sec:stat_tools}, \ref{sec:overview_outline}, \ref{sec:pt} and \ref{sec:discussion} for detailed changes, as well as our responses to R3O1-O3.


%\vspace{-0.15cm}
\section{Response to Reviewer 2}
\vspace{-0.5em}%\vspace{-0.1cm}

\begin{revcomment}{R2O1} \textit{``the introduction does not clearly explain that the proposed method is suitable for classification tasks''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will clarify in the introduction that our main focus is on classification, and will also discuss in future work how our approach can be extended to open-ended tasks.'' 

\noindent\textit{Revision Performed:} We have now discussed in the introduction that ``\rtwo{We focus on using LLMs for classification, specifically multiclass classification for AT queries and binary classification for PT and RT queries}'' and in the conclusion mention that ``\rtwo{We plan to extend \name{} to open-ended tasks which requires further consideration on how to calculate proxy scores}''.

\begin{revcomment}{R2O2} \textit{``the authors may want to evaluate the approach on Entity Matching ...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a discussion on how our work applies to entity resolution task as future work, and discuss other opportunities for optimization...'' 

\noindent\textit{Revision Performed:} Our revised conclusion section mentions that ``\rtwo{We plan to extend \name{} to \textit{semantic join} \cite{patel2024lotus} and entity matching operations which can be formulated as a filter on the cross product of two datasets. \name{} can be applied as is, but additional optimizations are possible by considering properties of the operations (e.g., transitivity in entity matching).}''


%\vspace{-0.15cm}
\section{Response to Reviewer 3}\label{sec:r3}
\vspace{-0.5em}
\begin{revcomment}{R3O1} \textit{``The paper introduces numerous variants of PRISM. To select the most appropriate variant ... include a summary table. ...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a table outlining various PRISM variants and their requirements and benefits.''

\noindent\textit{Revision Performed:} We have now added Sec.~\ref{sec:overview_outline} together with Table~\ref{tab:prism_variants} that outlines the main \name{} variants, their main parameters and their use-cases. We include the discussion here for ease of reference (please see the main paper for Table~\ref{tab:prism_variants}). 

\textit{In Sec.~\ref{sec:overview_outline}:} \rall{\overview{}}

%summarizes the \name{} variants with the aid of Table~\ref{tab:prism_variants} : ``\rall{Our main proposed \name{} variants for each of the queries are shown in Table~\ref{tab:prism_variants}. The variants in the table perform adaptive sampling; for ease of exposition, we also present other variants (not mentioned in the table) that perform uniform sampling. All variants take the quality target, $T$, and confidence parameter, $\delta$, as input, while \name{}$_P$-A and \name{}$_R$-A additionally require the oracle budget, $k$, upfront. All methods additionally use other internal hyperparameters which need not be set by the users and modifying their default values have limited impact on utility. We discuss how these parameters are set in Sec.~\ref{sec:hyperparam}}.'' In Sec.~\ref{sec:overview_outline}, we furthermore discuss the use-cases of \name{} variants: \rall{\name{}$_A$ is suitable for multi-class classification, as well as binary classification without a maximum oracle budget constraint but when the goal is to minimize the total budget used. \name{}$_P$ and \name{}$_R$ on the other hand respect a maximum oracle budget and thus are useful when user wants to stay within a budgetary constraint. Moreover,  \name{}$_P$ and \name{}$_R$ are useful for binary classification tasks with class imbalance, e.g., when there is expected to be few records in the positives class. Finally, \name{}$_A$-A and \name{}$_A$-M differ in that \name{}$_A$-A chooses a single cascade threshold for all output classes while \name{}$_A$-M chooses multiple cascade thresholds, one for each class. As such, \name{}$_A$-M is beneficial if the proxy is differently calibrated for different output classes, which for instance may occur if it is more difficult to correctly output one class but not another.}

%We present the discussion here as well for ease of reference.

%\textit{In Sec.~\ref{sec:overview_outline}:} \overview{}

\begin{revcomment}{R3O2} \textit{``Including a notation table would ... help readability...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a table of notation.''

\noindent\textit{Revision Performed:} We added a table of notation, see Table~\ref{tab:notation}.

\begin{revcomment}{R3O3}  \textit{``The paper frequently refers to external works and notations that are not self-contained within the text ...''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will include a brief description of the referenced statistical results up front.''


\noindent\textit{Revision Performed:} We have now added Sec.~\ref{sec:stat_tools} that discusses the referenced statistical results and discusses various parameters within them. This discussion now contains a simplified statement of the statistical results used from external work, which makes the paper more self-contained (see the newly added Lemma~\ref{lemma:hypothesis_test}). It furthermore provides a high-level intuition about the results, and provides a discussion of key terms in Lemma~\ref{lemma:hypothesis_test}: ``\rall{$\hat{\sigma}_i^2$ (resp., $\hat{\mu}_i$) is a term analogous to empirical variance (resp., mean). $\mathscr{K}(m, X)$, informally, quantifies whether the sequence of $X_i$ consistently exceeds $m$, when normalized by the variance $\hat{\sigma}_i^2$; larger values show observations exceed $m$ more frequently (thus suggesting $\mu>m$). The use of empirical variance $\hat{\sigma}_i^2$ contrasts with Hoeffding's inequality that only relies on the empirical mean. Taking standard deviation into account significantly improves the bounds when standard deviation is small, as our experiments show (see Sec.~\ref{sec:prec:unif} for comparison)}.'' We have additionally modified Sec.~\ref{sec:pt} and Sec.~\ref{sec:discussion} where the statistical tools are applied to refer back to Sec.~\ref{sec:stat_tools} to be more self-contained. More specifically, the definitions of $\mathscr{E}^{\text{\name{}}}$, $\mathscr{E}_A^{\text{\name{}}}$ and $\mathscr{E}_R^{\text{\name{}}}$, are now changed to refer to Lemma~\ref{lemma:hypothesis_test}. 

%We present the discussion here as well for ease of reference.

%\textit{In Sec.~\ref{sec:stat_tools}:} \stattools{}


\begin{revcomment}{R3M1.} \textit{``The figures in the paper are too small ... Improving the layout and scaling of the figures would ... enhance the presentation.''} 
\end{revcomment}

\noindent\textit{Proposed Revision Item:} ``We will enhance the layout and figures.''

\noindent\textit{Revision Performed:}  We have now split up figure in the introduction to improve the layout and scaling. 


